Cross-correlation effects in the solution NMR spectra of near-equivalent spin-1/2 pairs

The NMR spectra of spin-1/2 pairs contains four peaks, with two inner peaks much stronger than the outer peaks in the near-equivalence regime. We have observed that the strong inner peaks have significantly different linewidths, when measurements were performed on a 13C2-labelled triyne derivative. This linewidth difference may be attributed to strong cross-correlation effects. We develop the theory of cross-correlated relaxation in the case of near-equivalent homonuclear spin-1/2 pairs, in the case of a molecule exhibiting strongly anisotropic rotational diffusion. Good agreement is found with the experimental NMR lineshapes.

==> figures/4x4_relax_superop.tex <==
\begin{figure}[tbh] \label{relax_superop_plot}
\centering
\includegraphics[width=0.6\linewidth]{./graphics/relax_supermatrix.png}
\caption{ The \(\ (-1) \)-QC block of the real part of the Liouvillian in the \(\mathbb{B}_{Q}\) basis.
}
\label{fig:4x4_relax_superop_plot} 
\end{figure}

==> figures/P_D_L_frame_transformation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=2.1\linewidth]{./graphics/P_D_L_frame_transformation.png}
\caption{Coherences with spectrum}
\label{fig:P_D_L_frame_transformation} 
\end{figure}

==> figures/R2_vs_B0.tex <==
\begin{figure} \label{r2vsB0}
\centering
\includegraphics[width=1\linewidth]{./graphics/lambda_vs_b0.png}
    \caption{Plot of the decay rate constants \(\lambda_{\pm}\) against static field strength, \(B_{0}\). A minimum occurs for the rate constant \(\lambda_{+} = 0.085 \ \mathrm{s}^{-1}\) at \(B_{0} = 1.85 \ \mathrm{T}\), which is due to the partial cancellation of the DD and CSA mechanisms for the decay of the coherence 
    \(\big| |T_{0} \rangle \langle T_{+1} | \big)\) at this field.
    }
\label{fig:R2_vs_B0} 
\end{figure}

==> figures/experiment_and_simulated_spectra.tex <==
\begin{figure}[tbh]
\centering
\includegraphics[width=0.9\linewidth]{./graphics/experimental_and_simulated_spectra.png}
\caption{Experimental and simulated spectrum. The experimental spectrum is a simple pulse-acquire spectrum and is given by the filled line. The simulated spectrum is given by the dashed line and was simulated in the \textit{SpinDynamica} software package.}
\label{fig:triyne_experimental_simulated_spectrum} 
\end{figure}

==> figures/intermediate_2.tex <==
\begin{figure}[tbh]
\centering
\includegraphics[width=0.3\linewidth]{./graphics/intermediate_2.png}
\label{fig:intermediate_2} 
\end{figure}

==> figures/intermediate_3.tex <==
\begin{figure}[tbh]
\centering
\includegraphics[width=0.3\linewidth]{./graphics/intermediate_3.png}
\label{fig:intermediate_3} 
\end{figure}

==> figures/long_tau_lambda_vs_B0.tex <==
\begin{figure}[tbh] \label{relax_superop_plot}
\centering
\includegraphics[width=0.9\linewidth]{./graphics/long_tau_lambda_vs_B0.png}
\caption{  
}
\label{fig:long_tau_lambda_vs_B0} 
\end{figure}

==> figures/lorentzian_decomposition.tex <==
\begin{figure}[tbh]
\centering
\includegraphics[width=0.9\linewidth]{./graphics/lorentzian_decomposition.png}
\caption{lorentzian decomposition of spectrum.}
\label{fig:lorentzian_decomposition} 
\end{figure}

==> figures/relaxation_supermatrix_coherence_order.tex <==
\begin{figure}[tbh]
\centering
\includegraphics[width=0.6\linewidth]{./graphics/relaxation_supermatrix_coherence_order.png}
\caption{Relaxation supermatrix with a block-diagonal structure in coherence-order.}
\label{fig:relaxation_supermatrix_coherence_order} 
\end{figure}

==> figures/shifted_energy_levels.tex <==
\begin{figure}[tbh]
\centering
\includegraphics[width=0.95\linewidth]{./graphics/perturbed_eigenstates.png}
\caption{Shifted energy levels.}
\label{fig:perturbed_eigenstates} 
\end{figure}

==> figures/synthesis_of_I.tex <==
\begin{figure}[tbh]
\centering
\includegraphics[width=0.95\linewidth]{./graphics/synthesis_of_I.png}
\label{fig:synthesis_of_I} 
\end{figure}

==> figures/triyne_5.tex <==
\begin{figure}[tbh]
\centering
\includegraphics[width=0.5\linewidth]{./graphics/triyne_5.png}
\label{fig:triyne_5} 
\end{figure}

==> figures/triyne_experimental_spectrum.tex <==
\begin{figure}[tbh]
\centering
\includegraphics[width=0.9\linewidth]{./graphics/triyne_experimental_spectrum.pdf}
\caption{Experimental spectrum.}
\label{fig:triyne_experimental_spectrum} 
\end{figure}
